Style Transfer for Non-differentiable Audio Effects

Digital audio effects are widely used by audio engineers to alter the acoustic and temporal qualities of audio data. However, these effects can have a large number of parameters which can make them difficult to learn for beginners and hamper creativity for professionals. Recently, there have been a number of efforts to employ progress in deep learning to acquire the low-level parameter configurations of audio effects by minimising an objective function between an input and reference track, commonly referred to as style transfer. However, current approaches use inflexible black-box techniques or require that the effects under consideration are implemented in an auto-differentiation framework. In this work, we propose a deep learning approach to audio production style matching which can be used with effects implemented in some of the most widely used frameworks, requiring only that the parameters under consideration have a continuous domain. Further, our method includes style matching for various classes of effects, many of which are difficult or impossible to be approximated closely using differentiable functions. We show that our audio embedding approach creates logical encodings of timbral information, which can be used for a number of downstream tasks. Further, we perform a listening test which demonstrates that our approach is able to convincingly style match a multi-band compressor effect.

==> discussion.tex <==
\section{Limitations and Future Work}

\subsection{Limitations}

In the previous section, we addressed the three research questions we posed. In this section, we will explore the limitations of our style-matching model and evaluate the comprehensiveness of our analysis.

Overall, while our audio embedding network was able to separate DAFX classes and capture a number of perceptually relevant features, the end-to-end network had difficulty in utilising these embeddings for style matching, particularly with DAFX implementations outside of those that the model was trained on.

One major reason for this may be due to the inability for the audio encoder to separate the high-level timbral changes in effects from the content of the audio sources (i.e. different speakers, or musical content) under consideration. That is, the model has difficulties in identifying when similar settings are used for vastly different audio sources. This has obvious implications on the style-matching tasks which materialised in poor performance with unseen DAFX implementations. This may be due to the implementation of a single audio encoder for all effects, and may be mitigated by implementing separate encoders for relevant timbral features for different effect types (see discussion of future work in the following subsection).

% To ensure a more comprehensive evaluation of the latent controller, additional investigation may be required. This could involve recruiting more experts to conduct a similar evaluation as the one performed in Section \ref*{sec:latenteval}{}. Additionally, normalising user evaluation scores by taking into account their mean rating could provide a more equitable comparison for assessing the practical applicability of our low-dimensional latent controller.

Finally, this work could be improved by providing a similar MUSHRA test as performed in Section \ref{sec:mushra} for DAFX and audio data seen during training. This would provide both deeper insight into the metrics collected in Section \ref{sec:end2endeval}, as well as a comparison to the out-of-dataset MUSHRA test.

\subsection{Future Work}

In future work, we suggest revisiting the encoder network and examining the possible advantages of conditioning on the latent space and employing distinct encoders for DAFX classes. The latter can be achieved by training a classifier similar to that described in Section \ref{sec:audioencoder} to identify effect classes during style matching. Each umbrella DAFX class (e.g. temporal effects such as Ambience and Delay, or modulation effects such as Flanger or Leslie) could have its own trained audio encoder. This would encourage the encoder to learn features that are more specific to that particular class of effect.

% An approach for latent space regularisation would be to use perceptually-regulated variational timbre spaces as proposed by Esling et al. \citep{esling2018bridging}. This method would necessitate human-labeling of perceptually different DAFX settings. The induced topology of this perceptual space could then be used for regularisation during $\beta$-VAE training. That is, two audio sources with comparable DAFX settings applied should be mapped to nearby points in the timbral latent space. This may aid in strengthening the link between embeddings and high-level perceptual changes to \textit{effects}, rather than changes to audio sources.
